Multimodal Molecular Pretraining via Modality Blending

Self-supervised learning has recently gained growing interest in molecular modeling for scientific tasks such as AI-assisted drug discovery. Current studies consider leveraging both 2D and 3D molecular structures for representation learning. However, relying on straightforward alignment strategies that treat each modality separately, these methods fail to exploit the intrinsic correlation between 2D and 3D representations that reflect the underlying structural characteristics of molecules, and only perform coarse-grained molecule-level alignment. To derive fine-grained alignment and promote structural molecule understanding, we introduce an atomic-relation level "blend-then-predict" self-supervised learning approach, MoleBLEND, which first blends atom relations represented by different modalities into one unified relation matrix for joint encoding, then recovers modality-specific information for 2D and 3D structures individually. By treating atom relationships as anchors, MoleBLEND organically aligns and integrates visually dissimilar 2D and 3D modalities of the same molecule at fine-grained atomic level, painting a more comprehensive depiction of each molecule. Extensive experiments show that MoleBLEND achieves state-of-the-art performance across major 2D/3D molecular benchmarks. We further provide theoretical insights from the perspective of mutual-information maximization, demonstrating that our method unifies contrastive, generative (cross-modality prediction) and mask-then-predict (single-modality prediction) objectives into one single cohesive framework.

==> sections/intro-old.tex <==

\section{Introduction}

% \cm{introduction and importance of unlabeled molecular representation learning: fundamental challenge of drug discovery}

Artificial intelligence for drug discovery has garnered increasing interest in recent years~\cite{gomez2018automatic}. Among many challenges therein, self-supervised molecular representation learning, which extracts meaningful representations from large amounts of unlabeled molecules to serve as a solid \textit{foundation}~\cite{bommasani2021opportunities} for downstream molecular tasks, has become a critical and fundamental research problem for advancing drug discovery.
% The chemical space in which a drug candidate lies is vast, while drug-related labeled data is scarce and expensive to obtain. 


% \cm{introduce current representation learning methods, 2D, 3D}
\qy{I think this paragraph can be trimmed down, because uni-modal methods are not our focus.}
Molecules are typically represented as 2D topological graphs or 3D spatial structures, with most existing approaches focus on single modality. 2D molecular representation learning methods can be categorized into a) generative methods~\cite{hu2020strategies,rong2020self} that mask and reconstruct substructures, and b) contrastive methods~\cite{sun2020infograph,you2020graphcl,wang2022molclr} that learn invariant molecular graph representations.
Recent 3D pretraining methods demonstrate remarkable performance on molecular property prediction tasks, the core idea is to recover the corrupted 3D information, such as coordinates~\cite{zaidi2022pre,liu2022molecular,zhou2023uni,jiao2022energy}, atom types~\cite{zhou2023uni}, bond lengths and angles~\cite{fang2022geometry}.
% SMILES-BERT learns from 1D SMILES~\cite{wang2019smiles}, GROVER~\cite{rong2020self} learns from 2D topological graphs, and Uni-Mol~\cite{zhou2023uni} is a purely 3D molecular pretraining framework. 
% While each of these approaches has shown promise, combining multiple modalities may offer a more comprehensive representation of molecules and potentially improve the performance even further. Recently, there have been some attempts trying to incorporate 2D and 3D information~\cite{stark20223d}. However, the 3D positions only serve as auxiliary information to enhance 2D representations, and the models cannot accept 3D positions as input for 3D tasks.  and fail to leverage the potential complementary effect between different modalities

Recently, researchers have begun to investigate multimodal representation learning that leverages both 2D and 3D information~\cite{liu2022pre,stark20223d,liu2023molsde,luo2022one,zhu2022unified}, motivated by 1) the importance of 3D information in predicting molecular functionalities and enhancing 2D model performance~\cite{liu2022pre}, 2) pure 3D models are often infeasible for many real-world applications due to the computational complexity of calculating 3D geometry for large amounts of molecules~\cite{stark20223d}, making models able to process 2D input more practical and efficient.
% because explicitly computing 3D geometry for large amounts of molecules is computationally intractable, so models that can process 2D input offer practical advantages and efficiency.
Current methods, however, typically employ sample-level coarse-grained alignment strategies and encode two modalities separately. They rely on either contrastive learning with two separate models~\cite{liu2022pre,stark20223d,liu2023molsde}, or sample-level generative mutual prediction that processes 2D or 3D inputs separately~\cite{liu2022pre,zhu2022unified,liu2023molsde}. The latter can be considered a variant~\cite{liu2022pre} of BYOL~\cite{grill2020bootstrap} and SimSiam~\cite{chen2021exploring}, namely contrastive learning with asymmetric predictors for predicting one another for molecule-level alignment. Despite their utility, sample-level coarse-grained approaches have been found to lack structural and compositional understanding~\cite{yuksekgonul2022and}, and focus on global information while neglecting local structure details~\cite{xie2022revealing}. 
In addition, different modalities of a molecule essentially represent different manifestations of the same entity, while existing methods process inputs from different modalities separately, which is not conducive to the learning of unified molecular representations.

% Recent studies have explored multimodal representation learning, which combines both 2D and 3D information in molecular models. This approach is driven by the importance of 3D information for predicting molecular functionalities, and the challenges associated with using purely 3D models due to their computational complexity in real-world applications.

% In this work, we further propose that different modalities of molecules should be \textit{unified modeled} and comprehensively integrated with more thorough modality fusion.

In this work, we advocate for \textit{unified molecular modeling} with more comprehensive and fine-grained integration of modalities, by blending them together as input.
We introduce a higher level of abstraction for different molecular modalities, proposing to align manifolds at the finest granularity by leveraging shared entities across modalities as anchors, specifically, atom \textit{relationships}.
While modalities may appear distinct and reside in different high-dimensional spaces with unique manifolds (e.g., 2D shortest path, edge type, and 3D Euclidean distance), they all represent the same underlying entities—\textit{atoms} and their \textit{relationships}, at a higher level of abstraction. 
Consequently, we argue that information from various modalities should be unified and modeled together, rather than treated separately or with different models.
Distinct from existing works that explicitly distinguish different input modalities, we propose blending all modalities together as input within a single backbone model for thorough modality fusion, facilitating the unified modeling of different modalities.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/intro.pdf}
    \caption{TO be updated. This figure is to show 1) the modality-switching process, 2) versatility of the trained unified model}
    \label{fig:intro}
\end{figure}


% By doing so, we can capture the essential features of molecules more comprehensively.

% we can effectively model and analyze a wide range of molecules without incurring the computational overhead associated with 3D modeling.
% By unifying these modalities into a single modeling framework that captures the shared underlying structure, we can achieve more effective and efficient modeling of molecules in a variety of contexts.

% GPT-4
% In contrast to the majority of existing research, our study asserts that various molecular modalities should be integrated into a unified model for the following reasons:
% Although different modalities, such as 2D shortest path or edge type and 3D Euclidean distance, seem distinct and reside in separate spaces, they represent the same underlying entities at a higher level of abstraction—namely, atoms and their relationships. Consequently, we argue that information from these modalities should be combined and modeled collectively, rather than processed separately by distinct models. This holistic approach enables us to more comprehensively capture the essential features of molecules.
% 3D geometry is crucial for predicting molecular functionalities, and it should be incorporated into the model as it offers complementary and comprehensive information when compared to purely 2D models.
% Models capable of processing 2D input, in comparison to those limited to 3D input, provide practical advantages and increased efficiency in various contexts. This is particularly relevant when obtaining the 3D conformation of certain molecules proves difficult, as acquiring 3D equilibrium structures often necessitates costly DFT-based optimization.

We propose MOSS (MOdality-Switching\footnote{The term "switching" originates from a linguistic phenomenon known as "\href{https://en.wikipedia.org/wiki/Code-switching}{\textit{Code-switching}}".} \{Molecular representation learning / Auto-encoder / Self-supervised learning\} \{Towards Unified Molecular Modeling\}) \cm{TODO: a better name}, 
a self-supervised training algorithm towards unified molecular modeling.
We propose a fine-grained anchor-based alignment strategy that employs atom relationships as anchors to align the fundamentally identical yet seemingly dissimilar 2D and 3D manifolds at relation-level, in contrasting to existing methods that typically perform sample-level coarse-grained alignment. Our approach aims to learn unified representations that bind these two distinct manifolds into a shared space, allowing for modeling their intrinsic essential representations in a cohesive and unified manner.

Specifically, MOSS introduces a novel \textit{switch-then-predict} self-supervised learning method, consisting of two steps: modality-switching encoding and modality-specific prediction.
In modality-switching encoding, we switch and blend  atom relations from different modalities into a whole relation matrix without overlap, which is then fed into the model for unified encoding.
Notably, different from all existing methods, our model perceives different \textit{parts} of 2D \textit{and} 3D information, instead of receiving the \textit{whole} 2D \textit{or} 3D relations~\cite{liu2022pre,stark20223d,luo2022one,liu2023molsde,zhu2022unified}, which enables better cross-modal interaction and unified encoding, and further facilitates the creation of unified representations. 
In modality-specific prediction, the model is required to recover all modality-specific information separately.
We adopt shortest path distance and edge type~\cite{ying2021transformers,luo2022one}, as well as 3D euclidean distance as three different appearances of atom relations across 2D and 3D modalities. 
The model first receives blended relations and is then asked to recover each part separately, forcing it to capture the most essential and shared representation of molecules.

% We first blend different parts of these relations together and feed it into model for forward, then the model is asked to recover all of them separately.
% Given fused input and then predict each part separately will force the model to capture the most essential and shared representation of molecules.

By aligning the 2D and 3D manifolds, our unified trained model is versatile and can process both 2D and 3D inputs and handle all possible real-world scenarios (Figure~\ref{fig:intro}). The model can perform tasks effectively and efficiently when only 2D information is available, and can perform tasks more accurately when 3D information is obtained, with a unified single model. This is because the embedding space is shared between the two manifolds, and our approach promotes essential unified molecule modeling by capturing the most essential representation of molecules.

% By processing information from multiple modalities within a single backbone (shared parameters), the model can learn how to incorporate and utilize information from different modalities effectively.

% We will experiment on the Transformer-M~\cite{luo2022one} backbone, a variant of Transformer. The model architecture is shown in Figure~\ref{fig:transm}. Transformer-M has the capability to process both 2D graphs  and 3D conformation as input, where 2D topological information (Shortest Path Distance and Edge Type) and 3D spatial information (Euclidean Distance) are injected into the self-attention bias, allowing it to effectively model the relation between atoms. The distinction between 2D and 3D modalities is that they have different relation matrixs (with shape $N^2$, $N$ is the number of atoms).

Empirically, we demonstrate the proposed modality-switching method for learning unified molecular representation achieves state-of-the-art performance across a broad range of 2D and 3D benchmarks.
Theoretically, we provide a perspective from mutual-information maximization to probe the switch-then-predict process, showing that our method essentially unifies all existing contrastive or generative objectives into a simple and unified objective formulation.

% MOSS injects into a single encoder, unimodal downstream tasks can benefit from the implicit 3D or 2D knowledge even if there is no available.


% Self-supervised representation learning has revolutionized many AI areas, such as Natural Language Processing and Multimodal Learning (GPT-series~\cite{brown2020language,radford2019language,radfordimproving}), Computer Vision (MAE~\cite{he2022masked}, EVA-series~\cite{fang2022eva,fang2023eva}). The success of such paradigm stems from the learning of a general `foundation model'~\cite{bommasani2021opportunities} that encodes comprehensive knowledge from large amounts of unlabeled data, which can then serve as a strong `foundation' for various downstream applications. 
% This approach has proven particularly useful in scenarios where labeled data is scarce or expensive to obtain.

% \begin{table}[]
%     \centering
%     \begin{tabular}{l|cccccc}
%     \toprule
%     Methods & Tox21 $\uparrow$ & MUV $\uparrow$ & Bace $\uparrow$ & GAP $\downarrow$ & HOMO $\downarrow$ & LUMO $\downarrow$ \\ \midrule
%     VRR (GraphMVP) & 73.6 & 75.5 & 72.7 & 44.64 & 27.32 & 22.50 \\
%     SDE (MolSDE) & 75.6 & 80.1 & 79.0 & 42.75 & 25.84 & 21.52 \\ \midrule
%     MOSS & \textbf{78.68} & & \textbf{84.68} & \textbf{34.94} & \textbf{21.47} & \textbf{19.23} \\ \bottomrule
%     \end{tabular}
%     \caption{Performance comparison among purely generative pretraining. MOSS outperforms other generative methods by large margins across different kinds of benchmarks. MolSDE (ICML23) is the SoTA multimodal method released several days before submission.}
%     \label{tab:my_label}
% \end{table}

% Our contributions are three fold:

% \begin{itemize}
%     \item give an abstration of different modalities of molecules, and propose to leverage the commonly shared entities across modalities -- relations as anchors, to align two manifolds from the finest granularity.
%     \item We demonstrate that pure generative self-supervised learning can outperform methods that combine both contrastive and generative pretraining by a large margin, under the context that almost all multimodal methods emphasize the importance of contrastive learning to maximize the MI between different modalities. This should arise more thinking about molecular pretraining.
%     \item We present a simple and effective method towards unified and essential molecule modeling.
    
% \end{itemize}

